Dialogue Agents 101: A Beginner's Guide to Critical Ingredients for Designing Effective Conversational Systems

Sharing ideas through communication with peers is the primary mode of human interaction. Consequently, extensive research has been conducted in the area of conversational AI, leading to an increase in the availability and diversity of conversational tasks, datasets, and methods. However, with numerous tasks being explored simultaneously, the current landscape of conversational AI becomes fragmented. Therefore, initiating a well-thought-out model for a dialogue agent can pose significant challenges for a practitioner. Towards highlighting the critical ingredients needed for a practitioner to design a dialogue agent from scratch, the current study provides a comprehensive overview of the primary characteristics of a dialogue agent, the supporting tasks, their corresponding open-domain datasets, and the methods used to benchmark these datasets. We observe that different methods have been used to tackle distinct dialogue tasks. However, building separate models for each task is costly and does not leverage the correlation among the several tasks of a dialogue agent. As a result, recent trends suggest a shift towards building unified foundation models. To this end, we propose UNIT, a UNified dIalogue dataseT constructed from conversations of existing datasets for different dialogue tasks capturing the nuances for each of them. We also examine the evaluation strategies used to measure the performance of dialogue agents and highlight the scope for future research in the area of conversational AI.

==> tab_dataset.tex <==
\begin{table*}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\resizebox{\textwidth}{!}{%
\begin{tabular}{lp{10em}rp{10em}rrrrrrr}\toprule
\multirow{2}{*}{\textbf{Dataset}} &\multirow{2}{*}{\textbf{Description}} &\multirow{2}{*}{\textbf{Domain}} &\multirow{2}{*}{\textbf{Domain names}} &\multirow{2}{*}{\textbf{Dialogue History}} &\multirow{2}{*}{\textbf{External Knowledge}} &\multirow{2}{*}{\textbf{Output Format}} &\multicolumn{3}{c}{\textbf{Std Num Dialogues}} \\\cmidrule{8-10}
& & & & & & &\textbf{Train} &\textbf{Dev} &\textbf{Test} \\\midrule
CANARD &Dialogue rewriting, conversational search &Open &- &Multiple turns &None &Short text &4382 &489 &770 \\
CMU DoG &Document grounded dialogue &Open &- &Multiple turns &Unstructured text &Short text &3373 &229 &619 \\
ConvAI: Conversational intelligence &Knowledge grounded dialogue generation &Open &- &Multiple turns &None &Short text &2778 & & \\
ConvAI3: ClariQ &QA for open-domain information-seeking conversations &Open &- &Single turn and Multiple turns &Unstructured text &Short text &744869 &182435 & \\
CoQA &Question answering, generative question answering &7 &Children's stories, literature, mid/high school exams, news. wikipedia, reddit, science &Multiple turns &Unstructured text &Text span, short text &7199 &500 & \\
CoSQL &Dialogue state tracking &138 &Academic, Automobile, etc. &Multiple turns &None &Short text &2458 & & \\
DialoGLUE- Banking77 &Online banking queries &1 &Banking &Multiple turns &None &Short text &28176 &1540 &3080 \\
DialoGLUE- CLINC150 &Open intent discovery, intent classification &10 &Banking, work, meta, auto and commute, travel, home, utility, kitchen and dining, small talk, credit cards &Single turn &None &Short text &17250 &3000 &4500 \\
DialoGLUE- DSTC8 SGD &Multi-domain, task-oriented conversations between a human and a virtual assistant &4 &buses, events, homes, rental cars &Multiple turns &Structured schema &Short text &5525 &602 &1813 \\
DialoGLUE- HWU64 &Popular personal assistant queries &21 &alarm, audio, audiobook, calendar, cooking, datetime, email, game, general, IoT, lists, music, news, podcasts, general Q\&A, radio, recommendations, social, food takeaway, transport, weather &Single turn &None &Short text &9914 &1076 &1076 \\
DialoGLUE- MultiWOZ 2.1 &Multi-domain dialogues with multiple turns &7 &restaurant, hotel, attraction, taxi, train, hospital, police &Multiple turns &None &Short text &8438 &1000 &1000 \\
DialoGLUE- Restaurant8k &Restaurant booking domain queries &1 &Restaurant booking &Single turn &None &Short text &7968 &1000 &3731 \\
DialoGLUE- TOP &Compositional queries for hierachical semantic representations &2 &Navigation, events &Single turn &None &Short text &34406 &4462 &9042 \\
DialogSum &Summarization &Open &- &Multiple turns &None &Short text &12460 &500 &500 \\
Doc2Dial &Document grounded dialogue &4 &social security, veterans, dmv, student aid &Multiple turns &Unstructured text &Short text &3474 &661 &661 \\
MELD &Emotion classification &Open &- &Multiple turns &None &Short text &1037 &113 &279 \\
MUStARD &Sarcasm identification &Open &- &Multiple turns &None &Short text &690 & & \\
OTTers &One-turn topic transitions &Open &- &Multiple turns &Structured schema &Short text &1368 &774 &673 \\
PersonaChat &Personality driven conversations &Open &- &Multiple turns &Unstructured text &Short text &17878 &1000 & \\
ProsocialDialog &Respond to problematic content &Open &- &Multiple turns &Unstructured text &Short text &42304 &7132 &8701 \\
SAMSum Corpus &Summarization &Open &- &Multiple turns &None &Summary text &14731 &818 &819 \\
SPIDER &Semantic parsing, text-to-sql &138 &Academic, Automobile, etc. &Single turn &None &Short text &8659 &1034 & \\
Ubuntu Dialogue Corpus &Technical agent-user dialogues &1 &Technical &Multiple turns &None &Short text &1852868 & & \\
ABCD &Action-Based Conversations Dataset (ABCD) &1 &Online retail &Multiple turns &Meta data &Short text &8034 &1004 &1004 \\
bAbI &For automatic text understanding and reasoning &1 &Restaurant &Multiple turns &Structured schema &Short text &55441 &35933 &40968 \\
BiTOD &Bilingual multi-domain task oriented dialogues &5 &Attraction, metro, hotel, restaurant, weather &Multiple turns &Structured schema &Short text &2952 &295 &442 \\
CraiglistBargains &Strategic decision making &1 &Negotiation &Multiple turns &Meta data, image &Short text &5247 &597 &838 \\
DailyDialogue &Dialogue acts &Open &- &Multiple turns &None &Short text &11118 &1000 &1000 \\
DeliData &A dataset for deliberation in multi-party problem solving &Open &- &Multiple turns &None &Short text &500 & & \\
Empathetic Dialogues &For empathetic responses &Open &- &Multiple turns &None &Short text &17839 &2763 &2542 \\
FaithDial &Halucination free dialogues &Open &- &Multiple turns &Unstructured text &Short text &4094 &764 &791 \\
FusedChat &TOD and ODD fused dialogues &7 &restaurant, hotel, attraction, taxi, train, hospital, police &Multiple turns &None &Short text &10438 & & \\
mDIA &Multilingual dialogues &Open &- &Multiple turns &None &Short text &10000 &1000 &1000 \\
MetaLWOz &Meta learning WOz. Made for domain adaptation &47 &bus schedules, apartment search, alarm setting, banking, event reservation, etc &Multiple turns &None &Short text &37884 & & \\
Mutual &Multi turn dialogue reasoning &Open &- &Multiple turns &None &Short text &7088 &886 & \\
OpenDialKG &Explainable Conversational Reasoning with Attention-based Walks over Knowledge Graphs &4 &Movies, books, sports, music &Multiple turns &Unstructured text &Short text &13802 & & \\
SODA &Social dialogue dataset &Open &- &Multiple turns &Unstructured text &Short text &1191582 &146346 &148968 \\
Switchboard-1 &Telephonic conversations &Open &- &Multiple turns &None &Short text &1157 & & \\
Task2Dial &Commonsense enhanced Task-based Dialogue Grounded in Documents &1 &Cooking &Multiple turns &Unstructured text &Short text &357 & & \\
& & & & & & &1377533 &190588 &197553 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tab_tasks_intro.tex <==
\begin{table}[t]\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccp{20em}p{20em}}\toprule
\multicolumn{2}{c}{\textbf{Type}} &\textbf{Task} &\textbf{Dataset} \\\midrule

\multicolumn{1}{c|}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Generative}}}} &\multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Transformative}}}} &DR & CANARD \cite{elgohary-etal-2019-unpack} \\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &DS & SAMSum \cite{gliwa-etal-2019-samsum}, DialogSum \cite{chen-etal-2021-dialogsum}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &D2S & CoSQL \cite{yu-etal-2019-cosql}, SPIDER \cite{yu-etal-2018-spider}, TOP \cite{gupta-etal-2018-semantic-parsing}\\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & \\\cmidrule{2-4}

\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Response generation}}}} &QA & CMUDoG \cite{zhou-etal-2018-dataset}, CoQA \cite{reddy-etal-2019-coqa}, ClariQ \cite{aliannejadi2020convai3}, Mutual \cite{cui-etal-2020-mutual}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &KGR & ConvAI \cite{yusupov-kuratov-2018-nips}, Doc2Dial \cite{feng-etal-2020-doc2dial}, PersonaChat \cite{zhang-etal-2018-personalizing}, bAbI \cite{weston2015aicomplete}, FaithDial \cite{10.1162/tacl_a_00529}, OpenDialKG \cite{moon-etal-2019-opendialkg}, Task2Dial \cite{strathearn-gkatzia-2022-task2dial}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &CC & OTTers \cite{sevegnani-etal-2021-otters}, ProsocialDialog \cite{kim-etal-2022-prosocialdialog}, FusedChat \cite{Young_Xing_Pandelea_Ni_Cambria_2022}, mDIA \cite{zhang2022mdia}, SODA \cite{kim2022soda}, Switchboard-1 corpus \cite{Jurafsky-etal:1997}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &TOD & Ubuntu Dialogue Corpus \cite{lowe-etal-2015-ubuntu}, ABCD \cite{chen-etal-2021-action}, BiTOD \cite{lin2021bitod}, CraiglistBargains \cite{he-etal-2018-decoupling}, DeliData \cite{Karadzhov2021DeliDataAD}, MetalWOz \cite{shalyminov-etal-2019-shot} \\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & \\\midrule

\multicolumn{2}{c|}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Classification}}}} &ID & Banking77 \cite{casanueva-etal-2020-efficient}, CLINC150 \cite{larson-etal-2019-evaluation}, HWU64 \cite{Liu2021}, SGD Dataset \cite{Rastogi_Zang_Sunkara_Gupta_Khaitan_2020}\\

& \multicolumn{1}{c|}{} &SF & Restaurant8k \cite{coope-etal-2020-span}\\

& \multicolumn{1}{c|}{} &DST & MultiWOZ2.1 dataset \cite{eric-etal-2020-multiwoz}\\

& \multicolumn{1}{c|}{} &AD & MELD \cite{poria-etal-2019-meld}, DailyDialogue \cite{li-etal-2017-dailydialog}, MUStARD \cite{castro-etal-2019-towards}, Empathetic Dialogues \cite{rashkin-etal-2019-towards}\\

\bottomrule
\end{tabular}%
}
\caption{Dialogue tasks and corresponding datasets. Abbreviations -- DR: Dialogue Rewrite, DS: Dialogue Summary, D2S: Dialogue to Structure, QA: Question Answering, KGR: Knowledge Grounded Response, CC: Chit-chat, TOD: Task Oriented Dialogues, ID: Intent Detection, SF: Slot Filling, DST: Dialogue State Tracking, AD: Affect Detection.}
\label{tab:tasks_intro}
\vspace{-5mm}
\end{table}
